Mitigating Selection Bias with Node Pruning and Auxiliary Options

Large language models (LLMs) often exhibit systematic preferences for certain answer choices when responding to multiple-choice questions-a behavior known as selection bias. This bias reduces the accuracy and reliability of LLM outputs, limiting their usefulness in decision-critical applications. While prior work has focused on adjusting model inputs or outputs to mitigate this issue, our work takes a fundamentally different approach by identifying and removing the internal sources of bias. We introduce two methods: Bias Node Pruning (BNP), which prunes parameters that contribute to selection bias, and Auxiliary Option Injection (AOI), which introduces an additional answer choice to reduce bias in both white-box and black-box settings. To address the shortcomings of existing evaluation metrics, we propose Choice Kullback-Leibler Divergence (CKLD), a new metric that captures distributional imbalances in model predictions. Experiments on three LLMs across multiple datasets demonstrate that our methods consistently improve answer accuracy while reducing selection bias, providing a robust solution for both open- and closed-source models.

==> 2_ProblemStatement/metrics_notused.tex <==
\subsection{Bias Evaluation Metrics}
\label{sec:biasmetrics}
While the selection bias has been discussed in many previous works, its evaluation pipeline was rarely discussed in-depth.
Accordinlgy, in this section, we explain previous selection bias metrics, Standard Deviation of Recalls~(RStd) and Relative Standard Deviation~(RSD), and discuss their properties and limitations.
Then, we propose a new metric for selection bias evaluation dubbed \textit{Choice Kullback-Leibler Divergence}~(CKLD).

\input{C_Figures/metrics}
\textbf{Definition 1.} \textit{(Standard Deviation of Recalls) is the standard deviation of the class-wise recall:}
\begin{equation}
    \text{RStd} = \sqrt{\frac{1}{k}\sum_{i=1}^k(r_i - \bar{r})^2},
\end{equation}
\textit{where $k$ is the number of classes, $r_i$ is the recall of the $i$-th class, and $\bar{r}$ is the arithmetic mean of $r_i$ values.}~\citep{zheng2024large}

% \textbf{Property 1.1.} \textit{RStd is expected to be minimized at uniform prediction, $r_i = \frac{1}{k}$.}

% \textit{proof.} RStd is the standard deviation over the recall values for each class, and it is evident that it is minimized when $r_i = \bar{r}$ for $i = 1, \ldots, k$.
% To compute the expected value of $\bar{r}$, assume a $k$-way classification problem whose choice-wise labels and predictions are $y_i \in \mathbb{B}$ and  are $\hat{y}_i \in \mathbb{B}$ for $i = 1, \ldots, k$, respectively.
% Also, let their respective label proportion be $\{p_1, p_2, \ldots, p_k\}$, and the prediction proportion be $\{\hat{p}_1, \hat{p}_2, \ldots, \hat{p}_k\}$.
% Then, the expected recall for each class is
% \begin{equation}
%     \mathbb{E}[r_i] = P(\hat{y}_i = 1 \, | \, y_i = 1) = \hat{p}_i,
% \end{equation}
% where $i = 1, 2, \ldots, k$.
% Then, the expected value of $\bar{r}$ is
% \begin{equation}
%     \mathbb{E}[\bar{r}] = \mathbb{E}\big[\frac{1}{k} \sum_{i=1}^k \hat{p}_i\big] = \frac{1}{k}. 
% \end{equation}
% Thus, the RStd is expected to be minimized when predictions are uniform with ratio of $\frac{1}{k}$.
% \hfill $\square$



\textbf{Definition 2.} \textit{(Relative Standard Deviation) is the class-wise accuracy standard deviation normalized by the overall accuracy:}
\begin{equation}
    \text{RSD} = \frac{\sqrt{\frac{1}{k}\sum_{i=1}^k(s_i - \bar{s})^2}}{\bar{s}},
\end{equation}
\textit{where $k$ is the number of classes, $s_i$ is the accuracy of the $i$-th class, and $\bar{s}$ is the mean accuracy averaged across classes.}~\citep{croce2021robustbench, reif2024beyond}

In Figure~\ref{fig:metrics}, we empirically show how RStd and RSD behaves in different data setups.
Specifically, we vary the choice selection ratio (inner x axis) in different levels of label imbalance (outer x axis).
For instance, among four choices A$\sim$D with the proportion of label `A' being 0.55 with the other choices having 15$\%$ each, we plot how the metric values trend as the `A' prediction ratio is varied from 0.0 to 1.0.


The properties of each metric is empirically shown in Figure~\ref{fig:metrics}.
We tested the three metrics on a toy experiment setting with varying levels of label imbalance (outer x axis) and selection rates (inner x axis). 
Among four choices A$\sim$D with different `A' ratios (\textit{i.e.} if ratio is 0.55, 55$\%$ of the samples are labeled `A' and the rest of the samples are uniformly labeled), we plot the metrics' trend as the selection rate of choice A is varied.
RStd showed huge variance in its values, making it difficult to observe a trend.
We conjecture this is because RStd is not normalized like RSD.
RSD, on the other hand, showed a clear trend where its value is minimized when the `A' selection rate is 0.25.
This aligns with the Property 2.1 that the expected RSD is minimized at uniform prediction with probability $\frac{1}{4}$.
Finally, our CKLD showed the clearest trend where its value is minimized when the model's prediction rate is aligned with the label imbalance.
Also, CKLD had the lowest standard deviation overall, emphasizing its robustness in evaluation.

% \textbf{Property 2.1.} \textit{RSD is expected to be minimized at uniform prediction, $s_i = \frac{1}{k}$.}

% \textit{proof.} Assume the same scenario as in Property 1.1.
% Similarly,
% \begin{equation}
%     \mathbb{E}[s_i] = P(\hat{y}_i = y_i) =  \hat{p}_i,
% \end{equation}
% \begin{equation}
%     \mathbb{E}[\bar{s}] = \mathbb{E}\big[\frac{1}{k} \sum_{i=1}^k \hat{p}_i\big] = \frac{1}{k}. 
% \end{equation}
% Thus, the RSD is expected to be minimized when predictions are uniform with ratio of $\frac{1}{k}$.
% \hfill $\square$

% \textbf{Property 2.2.} \textit{RSD is always 0 in binary choice annotation tasks.}

% \textit{proof.} Assume a binary classification setting where labels are either `A' or `B'.
% In this setting, predicting `A' is analogous to predicting 'not B', and \textit{vice versa}.
% Therefore, accuracy of label `A' is identical to the accuracy of label `B', and the RSD value is always 0.
% \hfill $\square$


% While we lay a strong assumption that the labels and predictions are independent,
% % by computing the expectation within a random prediction scenario,
% it is important to note that the nature of RStd and RSD does not take label imbalance into account.
% % As both RStd and RSD metrics' expected minima is at uniform prediction of classes, class imbalance is not considered in the metrics.
% Hence, we propose Choice Kullback-Leibler Divergence~(CKLD), a new metric for bias evaluation which is sensitive to the ground-truth label proportion and applicable to all $k$-way classification tasks.

\textbf{Definition 3.} \textit{(Choice Kullback-Leibler Divergence) is the KL divergence between the ratio of each predicted choice and the ratio of each ground truth choice label:}
\begin{equation}
    \text{CKLD} = \sum_{i=1}^k \, p_i  \log{\frac{p_i}{q_i}},
\end{equation}
\textit{where $k$ is the number of classes, $p_i$ is the ratio of ground truth label choices, and $q_i$ is the ratio of each predicted choice label.}

% \textbf{Property 3.1.} \textit{CKLD is at minima when $p = q$.}

% \textit{proof.} (1) It is well known that KL divergence is non-negative, and
% (2) CKLD value is 0 when $p_i = q_i$.
% (3) Assume there exists a case where CKLD is 0 when $p_i \neq q_i$.
% CKLD is unique at this minima.

It is evident that CKLD reaches 0 when $p$ equals $q$, which is the minima of KL Divergence, and that CKLD is sensitive to label imbalance.
However, as CKLD does not take model performance (\textit{e.g.}, accuracy, recall, etc.) into consideration, it is important to refer to multiple metrics for robust assessment.
In this work, we leverage RSD and our CKLD metrics for selection bias evaluation.

\paragraph{Toy Experiments.} 
The properties of each metric is empirically shown in Figure~\ref{fig:metrics}.
We tested the three metrics on a toy experiment setting with varying levels of label imbalance (outer x axis) and selection rates (inner x axis). 
Among four choices A$\sim$D with different `A' ratios (\textit{i.e.} if ratio is 0.55, 55$\%$ of the samples are labeled `A' and the rest of the samples are uniformly labeled), we plot the metrics' trend as the selection rate of choice A is varied.
RStd showed huge variance in its values, making it difficult to observe a trend.
We conjecture this is because RStd is not normalized like RSD.
RSD, on the other hand, showed a clear trend where its value is minimized when the `A' selection rate is 0.25.
This aligns with the Property 2.1 that the expected RSD is minimized at uniform prediction with probability $\frac{1}{4}$.
Finally, our CKLD showed the clearest trend where its value is minimized when the model's prediction rate is aligned with the label imbalance.
Also, CKLD had the lowest standard deviation overall, emphasizing its robustness in evaluation.

% Relative Standard Deviation~(RSD) is a metric often adopted to evaluate fairness in classification problems~\citep{croce2021robustbench, reif2024beyond}.
% Compared to previous works that utilize class-wise accuracy, we employ the f1-score as the core performance measure.
% This is grounded on our finding that RSD$_\text{acc}$ is not applicable to binary classification tasks (\textit{i.e.} RSD$_\text{acc}$ is always 0 for binary classification tasks).


% However, a limitation of RSD$_\text{f1}$ is its insensitivity to label imbalance.
% Specifically, there are two key problems: (1) it is not necessarily at the minima when the distribution of selected choices matches that of the ground truth labels, and (2) it can exhibit sharp fluctuations when the distribution of predicted labels is extreme. 
% For instance, consider a binary classification task where $90\%$ of the ground truth labels are `A'. 
% Predicting `A' for $95\%$ of the samples results in a needlessly high RSD$_\text{f1}$ value, whereas CKLD would yield a more natural score that reflects the true label distribution, rendering a lower score that is closer to the minima. 
% This property of CKLD makes it valuable for ensuring fair assessments in datasets with significant class imbalances.



==> 2_ProblemStatement/prelim_old.tex <==


\subsection{Pilot study: Capturing Selection Bias}
\label{sec:pre_analysis}
§~\ref{sec:biasdef} shows that selection bias is prevalent in LLMs but not how it arises. This section presents two simple analyses to reveal how selection bias in represented in model embeddings and motivate our methods to reduce it.
%retrieve their embedding representations, motivating our method design.


\paragraph{Incorrect samples exhibit more selection bias.}
Figure~\ref{fig:pre_analysis}(a) shows the frequency of choices of the four response options on the ARC-Challenge dataset~\citep{clark2018think} using Llama-3-8B-Instruct~\citep{meta2024introducing} and Bloomz-7b1~\citep{muennighoff2023crosslingual}.
Ideally, if the models do not have selection bias, the choice frequency for each choice symbol should be near 0.25 given the ground-truth label ratios in Table~\ref{tbl:lbl_ratio} in Appendix~\ref{apdx:dataset}. 
However, the models show preferences for choice symbols `D' and `A', respectively.
This bias is more pronounced in cases where the models produce incorrect answers, highlighting the role of selection bias in model performance, and underscoring the importance of analyzing cases with incorrect model outputs.

\paragraph{Selection bias is prominently observed in the final decoder layers.}
To capture the selection bias, we investigate the difference between the correct and incorrect sample embeddings extracted from different locations.
Specifically, we explore the discrepancies within a single sample by permuting the sequence of choices in the question.
The difference between the embeddings within the choice-permuted set removes the sample-specific semantic information while the pure effect of the selection bias remains in the difference.


Accordingly, we first retrieve the intermediate embeddings of an LLM by computing the $t$-th token embedding from the $\ell$-th decoder layer as $\mathbf{z}_{\ell, t} = f_\ell(\mathbf{x}_\mathcal{A})_t$,
% \begin{equation}
%     \mathbf{z}_{\ell, t} = f_\ell(\mathbf{x}_\mathcal{A})_t, 
% \end{equation}
where $f_\ell$ is the LLM decoder up to the $\ell$-th layer and $\mathbf{x}_\mathcal{A}$ is the input with answer choices $\mathcal{A}$.
For brevity of notation, let $\mathbf{z} \in \mathbb{R}^d$ be the embedding from an arbitrary layer and token location.
Then, we quantify the selection bias by computing the embedding difference between the correct and incorrect questions within the permutations of $\mathcal{A}$.
That is, the bias vector $\mathbf{b}$ for a sample $\mathbf{x}$ is defined as
\begin{equation}
\label{eq:biasvec}
    \mathbf{b}_\mathbf{x} = \frac{1}{n_-} \sum_{i=1}^{n_-} \mathbf{z}_-^{(i)} \, - \, \frac{1}{n_+} \sum_{i=1}^{n_+} \mathbf{z}_+^{(i)},
    % \mathbf{b} = \frac{1}{|\mathcal{Z}|} \; \sum_{\{\mathbf{z}_-, \mathbf{z}_+\}\in \mathcal{Z}} \; \bigg[ \frac{1}{n_-} \sum_{i=1}^{n_-} \mathbf{z}_-^{(i)} \, - \, \frac{1}{n_+} \sum_{i=1}^{n_+} \mathbf{z}_+^{(i)} \bigg],
\end{equation}
where $\mathbf{z}_-$ is the embedding vector of the choice-permuted questions that the model answered incorrectly, and $\mathbf{z}_+$ is from the correctly answered questions.
Also, $n_-$ and $n_+$ correspond to the number of incorrect and correct questions, respectively.
% , so that $n_- + n_+$ equals the total number of possible permutations for each question.
To balance the number of correct and incorrect samples, we use the vector sets $\{\mathbf{z}_-, \mathbf{z}_+\}$ only when $1 \leq n_+ / n_- \leq 2$.
Then, we average the bias vectors across the samples in data subset $\mathcal{X}$ to define the average bias vector
\begin{equation}
\label{eq:avgbiasvec}
    \mathbf{b} = \frac{1}{|\mathcal{X}|} \sum_{\mathbf{x} \in \mathcal{X}} \mathbf{b}_\mathbf{x},
\end{equation}
where we use a subset size $|\mathcal{X}|$ of 32 in this work.
Refer to Figure~\ref{fig:main}(a) for visual aid.
% The effect of $\mathcal{X}$ size will be discussed later.

We use the L2 norm of the average bias vector retrieved from different layers and tokens as a proxy for the magnitude of selection bias. 
Figure~\ref{fig:pre_analysis}(b) shows the norm value from each location as a heatmap, where the x-axis lists the layer indices, and the y-axis shows the last 50 token embeddings of the inputs. 
The greater magnitude of the bias vector in the final layers motivates our approach in leveraging the interaction between the final embeddings and the linear output head.

% We use the L2 norm of the average bias vector to measure the level of bias in the embedding from a certain location (layer or token index).
% The values from each location is plotted as a heatmap in Figure~\ref{fig:pre_analysis} (b).
% Interestingly, the magnitude of the bias vector is prominent only in the last layer, motivating us to focus on the interaction of the bias vector with the output linear layer.


% \begin{equation}
%     \mathbf{b}_{\sigma(\mathcal{A})} = \mathbf{z}_{\sigma(\mathcal{A})} - \mathbf{z}_\mathcal{A},
% \end{equation}
% where $\sigma$ is an arbitrary permutation of the choices $\mathcal{A}$.
% Then, we take the expectation over all possible permutations to compute the bias vector
% \begin{equation}
%     \mathbf{b} = \mathbb{E}_{\sigma \in \mathfrak{S}}\big[\mathbf{z}_{\sigma(\mathcal{A})} - \mathbf{z}_\mathcal{A}\big],
% \end{equation}
% where $\mathfrak{S}$ is the set of all possible choice permutations.
% Since 
% However, since it is computationally expensive to average over all possible permutation pairs (\textit{e.g.}, there are $5! = 120$ permutations for a 5-way MCQ), we substitute average bias vector $\mathbf{b}$ with an alternative computation based on its correct
% \begin{equation}
% \label{eq:biasvec}
%     \mathbf{b} := \frac{1}{n_-} \sum_{i=1}^{n_-} \mathbf{z}_-^{(i)} \, - \, \frac{1}{n_+} \sum_{i=1}^{n_+} \mathbf{z}_+^{(i)},
% \end{equation}
% where $\mathbf{z}_-$ is the embedding vector among the choice-permuted questions that the model answered incorrectly, and $\mathbf{z}_+$ is from the correctly answered questions.
% Also, $n_-$ and $n_+$ each corresponds to the number of incorrect and correct questions.
% % , so that $n_- + n_+$ equals the total number of possible permutations for each question.
% To better capture the selection bias, we use the vector sets $\{\mathbf{z}_-, \mathbf{z}_+\}$ only when $1 \leq n_+ / n_- \leq 2$.

% % \begin{equation}
% % \label{eq:biasvec}
% %     \mathbf{b} := \frac{1}{|\mathcal{Z}|} \; \sum_{\{\mathbf{z}_-, \mathbf{z}_+\}\in \mathcal{Z}} \; \bigg[ \frac{1}{n_-} \sum_{i=1}^{n_-} \mathbf{z}_-^{(i)} \, - \, \frac{1}{n_+} \sum_{i=1}^{n_+} \mathbf{z}_+^{(i)} \bigg],
% % \end{equation}
% % where $\mathcal{Z}$ comprises the sets of all possible LLM output embeddings of the choice-permuted questions, $\mathbf{z}_-$ is the embedding vector of the choice-permuted questions that the model answered incorrectly, and $\mathbf{z}_+$ is from the correctly answered questions.
% % Also, $n_-$ and $n_+$ each corresponds to the number of incorrect and correct questions.
% % % , so that $n_- + n_+$ equals the total number of possible permutations for each question.
% % To better capture the selection bias, we use the vector sets $\{\mathbf{z}_-, \mathbf{z}_+\}$ only when $1 \leq n_+ / n_- \leq 2$.


% \input{B_Tables/early_exit}
% Then, we use the l2 norm of the average bias vector to measure the level of bias in the embedding from a certain location (layer or token index).
% The values from each location is plotted as a heatmap in Figure~\ref{fig:pre_analysis} (a).
% Interestingly, the magnitude of the bias vector is prominent only in the final layer, implicating a possible biased content in the output embeddings.
% However, when comparing the bias level of the responses retrieved from the final layer to those retrieved using the early-exit strategy~\cite{teerapittayanon2016branchynet}, responses from the penultimate layer did not have lower bias levels.
% This suggests



% An LLM that takes input $\mathbf{x}$ and predicts next token $\hat{\mathbf{y}}$ as
% \begin{equation}
% \begin{split}
%     \mathbf{z} &= \mathcal{F}(\mathbf{x})  \\
%     \hat{\mathbf{y}} &= h(\mathbf{z}),
% \end{split}
% \end{equation}
% where $\mathcal{F}$ is the decoder, $\mathbf{z}$ is the output hidden state of the final token, and $h$ is the linear head with softmax that maps the hidden states to the vocabulary space.
% We assume there exists a bias vector $\mathbf{b}$ that causes the permutation bias. 
% Then, we can debias the model by simply subtracting the bias vector from the hidden embedding as,
% \begin{equation}
% \begin{split}
%     \mathbf{z} &= \mathcal{F}(\mathbf{x}) \\
%     \hat{\mathbf{y}} &= h(\mathbf{z}  - \alpha \, \mathbf{b}),
% \end{split}
% \end{equation}
% where $\alpha$ is a hyperparameter that controls the effect of the bias embedding, whose bias embedding $\mathbf{b}$ is retrieved by
% \begin{equation}
%     \mathbf{b} = \mathbb{E}_{\{\mathbf{z}_-, \mathbf{z}_+\} \sim Z}\bigg[\frac{1}{n_-} \sum_{i=1}^{n_-} \mathbf{z}_-^{(i)} \, - \, \frac{1}{n_+} \sum_{i=1}^{n_+} \mathbf{z}_+^{(i)} \bigg],
% \end{equation}
% where $Z$ comprises the sets of all possible LLM output embeddings of the choice-permuted questions in the train set, $\mathbf{z}_-$ is the embedding vector of the choice-permuted questions that the model answered incorrectly, and $\mathbf{z}_+$ is from the correctly answered questions.
% Also, $n_-$ and $n_+$ each corresponds to the number of incorrect and correct questions, so that $n_- + n_+$ equals the total number of possible permutations for each question.
% To ensure the bias vector captures the information when the model is demonstrating permutation bias, we use the vector sets $\{\mathbf{z}_-, \mathbf{z}_+\}$ only when $1 \leq n_+ / n_- \leq 2$.


==> 3_Methods/aoi_old.tex <==
\subsection{Auxiliary Option Injection}
\label{sec:aoi}
Since selection bias is captured more when a model is incorrect, we hypothesized that providing an ``I don’t know”~(IDK) option would reduce selection bias. 
The auxiliary option $o_\text{aux}$ is applied as
\begin{equation}
    \mathcal{A} := \mathcal{A} \cup \{o_\text{aux}\}
\end{equation}
\begin{equation}
    \hat{\mathbf{a}} = \underset{{a \in \mathcal{A}\backslash o_\text{aux}}}{\arg\max} \; P(\hat{\mathbf{y}} = a \, | \, \mathbf{x}_\mathcal{A}),
\end{equation}
where $\mathcal{A}$ is the set of answer choices, and $\mathbf{x}_\mathcal{A}$ is the input question with choices $\mathcal{A}$.
How we retrieve the probability for each choice $a$ will be later discussed in the implementation details in §~\ref{sec:experiments} and Appendix~\ref{apdx:impdet}.
Further analyses on AOI will be provided in §~\ref{sec:aoi_anal}.




% \paragraph{Choice Delimiters (to be discussed in analysis.}
% Previous works have found that the Multiple Choice Symbol Binding~(MCSB) capability is crucial for the LLM to correctly respond to Multiple Choice Questions~\cite{robinson2023leveraginglargelanguagemodels,xue2024strengthened}. 
% Intuitively, we hypothesize this property will be enforced when each choice is clearly differentiated with other choices.
% Accordingly, we pre-pend an appropriate delimiter character to explicitly tell the model where each answer choice begins in the input question.
% We discuss the impact of different delimiters and the relationship between their length and its debiasing capabilities in section~\ref{}.

==> 3_Methods/bias_pruning_old.tex <==
\subsection{Bias Node Pruning}

As shown in §~\ref{sec:pre_analysis}, the average bias vector $\mathbf{b} \in \mathbb{R}^d$ is most prominent in the final layer, and the selection bias materializes in the final output projection parameters, $\bm{W} \in \mathbb{R}^{d \times |\mathcal{V}|}$, where $\mathcal{V}$ is the vocabulary set.
To mitigate the selection bias problem induced by the linear layer, we prune the parameters in $\bm{W}$ that contribute to the bias.
In choosing which parameters to prune, we gain intuition by approximating a biased model, $\mathcal{F}$, as
\begin{equation}
    \mathcal{F}(\mathbf{x}_\mathcal{A}) \approx (\mathcal{D}(\mathbf{x}_\mathcal{A}) + \mathbf{b})\cdot \bm{W},
\end{equation}
where $\mathcal{D}$ is a conceptual LLM decoder with zero selection bias, and $\mathbf{b}$ is the average bias vector defined in \eqref{eq:avgbiasvec}.
Then, $\mathbf{b} \cdot \bm{W}$ is the factor that contributes to the selection bias, and removing the parameters in $\bm{W}$ that has the most active interaction with $\mathbf{b}$ will reduce selection bias.
Accordingly, we choose the top-$k$ rows in $\bm{W}$ with respect to
\begin{equation}
\label{eq:topk}
    \mathcal{K} = \underset{i \in [1,d]}{\text{Top-}k} \; \bigg(\sum_{j=1}^{|\mathcal{V}|} \;\mathbf{b}_i \times \bm{W}_{ij}\bigg),
\end{equation}
where $|\mathcal{V}|$ is the vocabulary size of the output.
Then, we use the index in $\mathcal{K}$ to zero out the corresponding rows (\textit{i.e.}, nodes) in $\bm{W}$.
Bias Node Pruning~(BNP) is a one-time process with the average bias vector $\mathbf{b}$ being pre-computed, and the pruned weight $\tilde{\bm{W}}$ is applied to all test samples as $f(\mathbf{x}_\mathcal{A}) \cdot \tilde{\bm{W}}$ where $f$ is the LLM decoder.
Refer to Appendix~\ref{apdx:complexity} for complexity analysis.
Another design choice would deduct $\mathbf{b}$ from the decoder output embedding; however, we observed more stable performance by pruning the parameters in $\bm{W}$.

% In choosing which parameters to prune, we gain intuition by approximating the selection bias in \eqref{eq:sel_bias} as
% \begin{equation}
% \begin{split}
%     \mathbb{E}_{\sigma \in \mathfrak{S}}\big[\mathcal{F}(\mathbf{x}_{\sigma(\mathcal{A})})\big] - \mathcal{F}(\mathbf{x}_\mathcal{A}) \; &= \; \mathbb{E}_{\sigma \in \mathfrak{S}}\big[ (f(\mathbf{x}_{\mathcal{A}}) + \alpha \mathbf{b}) \cdot \bm{W} \big] - f(\mathbf{x}_\mathcal{A}) \cdot \bm{W}\\ \; &= \; \mathbb{E}_{\sigma \in \mathfrak{S}}\big[\mathbf{b}_{\sigma(\mathcal{A})}\big]\cdot \bm{W} \;\; = \;\; \mathbf{b} \cdot \bm{W},
% \end{split}
% \end{equation}
% % \begin{equation}
% % \begin{split}
% %     \mathbb{E}_{\sigma \in \mathfrak{S}}\big[\mathcal{F}(\mathbf{x}_{\sigma(\mathcal{A})})\big] - \mathcal{F}(\mathbf{x}_\mathcal{A}) \; &= \; \mathbb{E}_{\sigma \in \mathfrak{S}}\big[ (f(\mathbf{x}_{\mathcal{A}}) + \mathbf{b}_{\sigma(\mathcal{A})}) \cdot \bm{W} \big] - f(\mathbf{x}_\mathcal{A}) \cdot \bm{W}\\ \; &= \; \mathbb{E}_{\sigma \in \mathfrak{S}}\big[\mathbf{b}_{\sigma(\mathcal{A})}\big]\cdot \bm{W} \;\; = \;\; \mathbf{b} \cdot \bm{W},
% % \end{split}
% % \end{equation}

% where $\mathcal{F}$ is the LLM, $f$ is the decoder, $\mathbf{x}_{\sigma(\mathcal{A})}$ is the input prompt with one of the permutations of choice options $\mathcal{A}$, and $\mathbf{b}$ is the average bias vector defined in \eqref{eq:biasvec}.
% That is, $\mathbf{b} \cdot \bm{W}$ is the factor that contributes to the selection bias, and removing the parameters in $\bm{W}$ that has the most active interaction with $\mathbf{b}$ will reduce selection bias.
% Accordingly, we choose the top-$k$ rows in $\bm{W}$ with respect to
% \begin{equation}
%     \mathcal{K} = \underset{i \in [1,d]}{\text{Top-}k} \; \bigg(\sum_{j=1}^{|\mathcal{V}|} \;\mathbf{b}_i \times \bm{W}_{ij}\bigg),
% \end{equation}
% where $|\mathcal{V}|$ is the vocabulary size of the output.
% Then, we use the index in $\mathcal{K}$ to zero out the corresponding rows (\textit{i.e.}, nodes) in $\bm{W}$.
% Overall, Bias Node Pruning~(BNP) is a one-time process with the average bias vector $\mathbf{b}$ being pre-computed, and the pruned weight $\tilde{\bm{W}}$ is applied to all test samples as $f(\mathbf{x}) \cdot \tilde{\bm{W}}$.



==> 4_Experiments/blackbox_old.tex <==
\subsection{Black-box Settings}
\label{sec:blackbox}
Several state\--of\--the\--art models are black-box and their parameters are not open to the public.
In these cases, BNP is not feasible, leaving AOI as the only available technique for debiasing the model, using text outputs for prediction.
% For this reason, we devise a comparative experiment where only AOI is applied to the models.
For each model, including open-source LLMs~(\textit{e.g.} Llama-3, Bloomz, and Mistral) and closed-source LLMs~(\textit{e.g.}, Claude-3 Haiku and Sonnet models~\citep{anthropic2024introducing}), we generate text responses with the same input prompt.
Then we compute the Jaccard similarity between each choice option and the output text to select the choice with the highest similarity score, instead of the probability-based answer selection method used in our main experiments.
% This approach simulates a black-box setting with the white-box models.
% Moreover, we extend our experiment to Claude-3 Haiku and Sonnet models~\citep{anthropic2024introducing}, which are closed-source black-box models.
In Table~\ref{tbl:blackbox}, AOI generally improves black-box model performance (accuracy and F1) and reduces selection bias (RSD and CKLD).

==> 4_Experiments/evaluation_bak.tex <==

There is no consensus in the literature on how to measure selection bias.
Here, we first review two selection bias metrics, Standard Deviation of Recalls~(RStd) and Relative Standard Deviation~(RSD), which evaluate the consistency of \textit{performance} across choices.
By scrutinizing their limitations, we propose \textbf{Choice Kullback-Leibler Divergence}~(CKLD), which is a novel \textit{distribution}-based bias metric.

\textbf{Definition 1.} \textit{(Standard Deviation of Recalls) is the standard deviation of the class-wise recall:}
\begin{equation}
    \text{RStd} = \sqrt{\frac{1}{k}\sum_{i=1}^k(r_i - \bar{r})^2},
\end{equation}
\textit{where $k$ is the number of choices, $r_i$ is the recall of the $i$-th class, and $\bar{r}$ is the arithmetic mean of $r_i$ values}~\citep{zheng2024large}.

% \textbf{Property 1.1.} \textit{RStd is expected to be minimized at uniform prediction, $r_i = \frac{1}{k}$.}

% \textit{proof.} RStd is the standard deviation over the recall values for each class, and it is evident that it is minimized when $r_i = \bar{r}$ for $i = 1, \ldots, k$.
% To compute the expected value of $\bar{r}$, assume a $k$-way classification problem whose choice-wise labels and predictions are $y_i \in \mathbb{B}$ and  are $\hat{y}_i \in \mathbb{B}$ for $i = 1, \ldots, k$, respectively.
% Also, let their respective label proportion be $\{p_1, p_2, \ldots, p_k\}$, and the prediction proportion be $\{\hat{p}_1, \hat{p}_2, \ldots, \hat{p}_k\}$.
% Then, the expected recall for each class is
% \begin{equation}
%     \mathbb{E}[r_i] = P(\hat{y}_i = 1 \, | \, y_i = 1) = \hat{p}_i,
% \end{equation}
% where $i = 1, 2, \ldots, k$.
% Then, the expected value of $\bar{r}$ is
% \begin{equation}
%     \mathbb{E}[\bar{r}] = \mathbb{E}\big[\frac{1}{k} \sum_{i=1}^k \hat{p}_i\big] = \frac{1}{k}. 
% \end{equation}
% Thus, the RStd is expected to be minimized when predictions are uniform with ratio of $\frac{1}{k}$.
% \hfill $\square$


\textbf{Definition 2.} \textit{(Relative Standard Deviation) is the class-wise accuracy standard deviation normalized by the overall accuracy:}
\begin{equation}
    \text{RSD} = \frac{\sqrt{\frac{1}{k}\sum_{i=1}^k(s_i - \bar{s})^2}}{\bar{s}},
\end{equation}
\textit{where $k$ is the number of choices, $s_i$ is the accuracy of the $i$-th class, and $\bar{s}$ is the mean accuracy averaged across classes}~\citep{croce2021robustbench, reif2024beyond}.


% We applied each measure to a synthetic MCQ dataset (Figure 4). We constructed this data set by varying the choice selection ratio (inner x axis) under different ground-truth ratios (outer x axis). 
% For instance, in the third column of Figure 4, labelled ‘A’ Label Ratio 0.55, answer choice ‘A’ is the correct choice in 55 of the samples; in the remaining questions, the correct answer is ‘B’, ‘C’, or ‘D’ 15 of the time, respectively. 
% To simulate realistic predictions, we have the model render correct predictions half of the time, and predict randomly with respect to the choice selection ratio for the other half. 
% The choice selection ratio depends on the ‘A’ selection rate, e.g., if ‘A’ Selection Rate is 0.4, each choice will be sampled with respect to P (A) = 0.4 and P (B) = P (C) = P (D) = 0.2. With this set up, the selection bias metrics (vertical axis) should be lowest at the XXX, shown with a vertical dashed line in Figure 4.  


We empirically show how these performance-based metrics, RStd and RSD, behave across different data characteristics.
We constructed synthetic 4-way MCQ datasets by varying the choice selection ratio under different ground-truth ratios.
For instance, in the third column of Figure~\ref{fig:metrics}, labeled ```A' Label Ratio = 0.55", answer choice ‘A’ is the correct choice in 55$\%$ of the samples and the rest are labeled `B', `C', or `D' 15$\%$ of the time, respectively.
To simulate realistic predictions, we have the model render correct predictions half of the time, and predict with respect to the choice selection ratio (\textit{i.e.}, `A' selection rate) for the other half.
For example, if `A' Selection Rate is 0.4, each choice will be sampled with respect to $P(A) = 0.4$ and $P(B) = P(C) = P(D) = 0.2$ half of the time, and will predict the correct answer for the other half.
% The choice selection ratio is varied from 0.05 to 0.95 to plot each graph in Figure~\ref{fig:metrics}.
With this set up, the selection bias metrics should be lowest at the `A' Label Ratio, shown with a vertical dashed line in Figure~\ref{fig:metrics}.  

In contrast, the minimum points of RStd and RSD are not in the expected locations (Figure~\ref{fig:metrics}). 
Both metrics are insensitive to the ground-truth ratios. (RSD is lowest when the `A' Selection Rate is $\frac{1}{\text{\# Choices}} = \frac{1}{4}$ regardless of the `A' Label Ratio.) These results highlight the inability of RStd and RSD to measure selection bias in datasets with skewed distributions of the correct label.
% both metrics do not properly reflect label imbalance, highlighting the potential failure in evaluating datasets with skewed label distributions.
Therefore, we propose Choice Kullback-Leibler Divergence~(CKLD), a distribution-based metric sensitive to data distribution and imbalance of choice labels.

\textbf{Definition 3.} \textit{(Choice Kullback-Leibler Divergence) is the KL divergence between the ratio of each predicted choice and the ratio of each ground truth choice label:}
\begin{equation}
\label{eq:ckld}
    \text{CKLD} = \sum_{i=1}^k \, p_i  \log{\frac{p_i}{q_i}},
\end{equation}
\textit{where $k$ is the number of choices, $p_i$ is the ratio of ground truth label choices, and $q_i$ is the ratio of each predicted choice label.}


\input{C_Figures/metrics}

% \textbf{Property 3.1.} \textit{CKLD is at minima when $p = q$.}

% \textit{proof.} (1) It is well known that KL divergence is non-negative, and
% (2) CKLD value is 0 when $p_i = q_i$.
% (3) Assume there exists a case where CKLD is 0 when $p_i \neq q_i$.
% CKLD is unique at this minima.

CKLD is minimized when the predictions match the ground-truth ratio without bias towards certain choices (bottom row of Figure~\ref{fig:metrics}; proof in Appendix~\ref{apdx:proof} and further discussion in Appendix~\ref{apdx:ckld_discussion}).
However, CKLD does not account for the model performance in downstream tasks. Hence, it is important to refer to multiple metrics for a robust assessment.
In this work, we leverage both RSD and our CKLD metrics to evaluate selection bias.
We chose RSD because the groundtruth ratios of the benchmark datasets are close to uniform, and we can expect RSD to be minimized when the predictions are uniform. 

% It is evident that CKLD reaches 0 when $p$ equals $q$, which is the minima of KL Divergence, and that CKLD is sensitive to label imbalance.
% However, as CKLD does not take model performance (\textit{e.g.}, accuracy, recall, etc.) into consideration, it is important to refer to multiple metrics for robust assessment.
% In this work, we leverage RSD and our CKLD metrics for selection bias evaluation.

% \paragraph{Toy Experiments.} 
% The properties of each metric is empirically shown in Figure~\ref{fig:metrics}.
% We tested the three metrics on a toy experiment setting with varying levels of label imbalance (outer x axis) and selection rates (inner x axis). 
% Among four choices A$\sim$D with different `A' ratios (\textit{i.e.} if ratio is 0.55, 55$\%$ of the samples are labeled `A' and the rest of the samples are uniformly labeled), we plot the metrics' trend as the selection rate of choice A is varied.
% RStd showed huge variance in its values, making it difficult to observe a trend.
% We conjecture this is because RStd is not normalized like RSD.
% RSD, on the other hand, showed a clear trend where its value is minimized when the `A' selection rate is 0.25.
% This aligns with the Property 2.1 that the expected RSD is minimized at uniform prediction with probability $\frac{1}{4}$.
% Finally, our CKLD showed the clearest trend where its value is minimized when the model's prediction rate is aligned with the label imbalance.
% Also, CKLD had the lowest standard deviation overall, emphasizing its robustness in evaluation.

==> 4_Experiments/evaluation_old.tex <==
\subsection{Evaluation Metrics}
\label{sec:eval}


There is no consensus in the literature on how to measure selection bias.
Brute-force metrics like Proportion of Plurality Agreement~\cite{robinson2023leveraginglargelanguagemodels}, Permutation Sensitivity~\cite{liusie2024teacher}, and Fluctuation Rate~\cite{wei2024unveiling} directly compute the bias level using actual choice permutations.
Other metrics, like Standard Deviation of Recalls~(RStd; \citet{zheng2024large}) and Relative Standard Deviation~(RSD; \citet{croce2021robustbench}), compute the consistency of model performance across choices.
Considering the amount of computation that brute-force metrics require, we utilize the performance-based metrics in this work.
In particular, we adopt the RSD metric, defined as:

\paragraph{Definition 1.} \textit{(Relative Standard Deviation) is the class-wise accuracy standard deviation normalized by the overall accuracy:}
\begin{equation}
    \text{RSD} = \frac{\sqrt{\frac{1}{k}\sum_{i=1}^k(s_i - \bar{s})^2}}{\bar{s}},
\end{equation}
\textit{where $k$ is the number of choices, $s_i$ is the accuracy of the $i^{th}$ class, and $\bar{s}$ is the mean accuracy averaged across classes}~\citep{croce2021robustbench, reif2024beyond}.

Additionally, we introduce the Choice Kullback-Leibler Divergence~(CKLD) metric as a new distribution-wise perspective of selection bias evaluation.


\paragraph{Definition 2.} \textit{(Choice Kullback-Leibler Divergence) is the KL divergence between the ratio of each predicted choice and the ratio of each ground truth choice label:}
\begin{equation}
\label{eq:ckld}
    \text{CKLD} = \sum_{i=1}^k \, p_i  \log{\frac{p_i}{q_i}},
\end{equation}
\textit{where $k$ is the number of choices, $p_i$ is the ratio of ground truth label choices, and $q_i$ is the ratio of each predicted choice label.}

This metric is designed to be sensitive to choice symbol distributions, which is not directly captured in previous metrics.
That is, CKLD is minimized when the predictions match the ground-truth ratio without bias towards certain choices~(proof in Appendix~\ref{apdx:proof}).

In this work, we leverage both RSD and our CKLD metrics for comprehensive evaluation.
In addition to selection bias evaluation metrics, we also adopt Accuracy and F1 score to evaluate question-answering performance.
Full discussion on the choice of evaluation metrics is provided in Appendix~\ref{apdx:metrics} and Appendix~\ref{apdx:eda_metric}.

% Here, we first review two selection bias metrics, Standard Deviation of Recalls~(RStd) and Relative Standard Deviation~(RSD), which evaluate the consistency of \textit{performance} across choices.
% By scrutinizing their limitations, we propose \textbf{Choice Kullback-Leibler Divergence}~(CKLD), which is a novel \textit{distribution}-based bias metric.

% \textbf{Definition 1.} \textit{(Standard Deviation of Recalls) is the standard deviation of the class-wise recall:}
% \begin{equation}
%     \text{RStd} = \sqrt{\frac{1}{k}\sum_{i=1}^k(r_i - \bar{r})^2},
% \end{equation}
% \textit{where $k$ is the number of choices, $r_i$ is the recall of the $i$-th class, and $\bar{r}$ is the arithmetic mean of $r_i$ values}~\citep{zheng2024large}.



% \textbf{Definition 2.} \textit{(Relative Standard Deviation) is the class-wise accuracy standard deviation normalized by the overall accuracy:}
% \begin{equation}
%     \text{RSD} = \frac{\sqrt{\frac{1}{k}\sum_{i=1}^k(s_i - \bar{s})^2}}{\bar{s}},
% \end{equation}
% \textit{where $k$ is the number of choices, $s_i$ is the accuracy of the $i$-th class, and $\bar{s}$ is the mean accuracy averaged across classes}~\citep{croce2021robustbench, reif2024beyond}.




% We empirically show how these performance-based metrics, RStd and RSD, behave across different data characteristics.
% We constructed synthetic 4-way MCQ datasets by varying the choice selection ratio under different ground-truth ratios.
% For instance, in the third column of Figure~\ref{fig:metrics}, labeled ```A' Label Ratio = 0.55", answer choice ‘A’ is the correct choice in 55$\%$ of the samples and the rest are labeled `B', `C', or `D' 15$\%$ of the time, respectively.
% To simulate realistic predictions, we have the model render correct predictions half of the time, and predict with respect to the choice selection ratio (\textit{i.e.}, `A' selection rate) for the other half.
% For example, if `A' Selection Rate is 0.4, each choice will be sampled with respect to $P(A) = 0.4$ and $P(B) = P(C) = P(D) = 0.2$ half of the time, and will predict the correct answer for the other half.
% % The choice selection ratio is varied from 0.05 to 0.95 to plot each graph in Figure~\ref{fig:metrics}.
% With this set up, the selection bias metrics should be lowest at the `A' Label Ratio, shown with a vertical dashed line in Figure~\ref{fig:metrics}.  

% In contrast, the minimum points of RStd and RSD are not in the expected locations (Figure~\ref{fig:metrics}). 
% Both metrics are insensitive to the ground-truth ratios. (RSD is lowest when the `A' Selection Rate is $\frac{1}{\text{\# Choices}} = \frac{1}{4}$ regardless of the `A' Label Ratio.) These results highlight the inability of RStd and RSD to measure selection bias in datasets with skewed distributions of the correct label.
% % both metrics do not properly reflect label imbalance, highlighting the potential failure in evaluating datasets with skewed label distributions.
% Therefore, we propose Choice Kullback-Leibler Divergence~(CKLD), a distribution-based metric sensitive to data distribution and imbalance of choice labels.

% \textbf{Definition 3.} \textit{(Choice Kullback-Leibler Divergence) is the KL divergence between the ratio of each predicted choice and the ratio of each ground truth choice label:}
% \begin{equation}
% \label{eq:ckld}
%     \text{CKLD} = \sum_{i=1}^k \, p_i  \log{\frac{p_i}{q_i}},
% \end{equation}
% \textit{where $k$ is the number of choices, $p_i$ is the ratio of ground truth label choices, and $q_i$ is the ratio of each predicted choice label.}



==> 4_Experiments/mainexp_old.tex <==
\subsection{Experimental Results}
\label{sec:mainexp}

\paragraph{BNP + AOI consistently improves base model performance by reducing selection bias.}
Table~\ref{tbl:main} shows the performance of our methods with three LLMs and MCQ datasets.
For all models and data sets, BNP and/or AOI increased accuracy and F1 score and decreased RSD and CKLD.
It is especially noteworthy that Llama-3's accuracy on ARC-Challenge improves from 52.3$\%$ to 65.3$\%$ when both BNP and AOI are applied, an outstanding 24.9$\%$ increase.


\paragraph{Our method can be applied together with other debiasing and decoding methods.}
For further insight, we compare our methods with other debiasing and decoding approaches: Chain-of-Thought~(CoT; \cite{wei2022chain}), In-Context Learning~(ICL; \cite{brown2020language}), and Decoding by Contrasting Layers~(DoLa; \cite{chuang2023dola}).
For CoT, we follow the implementation of OpenAI Evals~\citep{OpenAIEvals} by first prompting with ``Let's think step by step", and then using the generated explanation to regenerate the final prediction.
In the case of ICL, we take one question from the training set to retrieve $N!$ choice-permuted questions, where $N$ is the number of choices.
Then, we randomly select three questions from the choice-permuted pool and create demonstrative examples from them, where the LLM agent always answers the choice-permuted questions correctly.
% Finally, we adopt the method of \cite{zheng2024large} for Calibration by retrieving the prior probability to debias the output.
Concrete prompt formats and details are provided in Appendix~\ref{apdx:baselines}. These baseline methods can be used along with our debiasing methods.
Both question answering and debiasing improve when our methods are applied together (Table~\ref{tbl:baselines}), even achieving the best performance in collaboration with appropriate baselines.
Note that the values denoted with `$*$' are measured only when our BNP is applied because AOI did not fare well in those cases.

==> 5_Analyses/aoi.tex <==
% \subsection{Analyzing Auxiliary Option Injection}
% \label{sec:aoi_anal}
% \input{B_Tables/aoi_ablation}

% \paragraph{Content of the auxiliary option matters.}
% Our experiments above used ``I don’t know'' as the auxiliary option, but other options are also possible. 
% We conducted an experiment where we substituted it with ``None of the above'' and ``I know the answer''.
% In Table~\ref{tbl:aoi_anal}, ``None" refers to the former, and ``Know'' refers to the latter type of auxiliary option.
% For Llama-3 and Bloomz, the inclusion of an auxiliary option improves performance and reduces selection bias relative to the baseline (Table~\ref{tbl:aoi_anal}), but the ``I don’t know'' (Ours) performs better in most cases.
% % When we compared `Model + Arbitrary' with `Model + Ours' on MMLU, we found that `Model + Arbitrary' does not outperform our proposed method. 
% % However, it still demonstrated gains in performance compared to the baseline Llama-3 model.
% With the Mistral model, however, the "I know the answer'' option degrades model performance and increases selection bias.
% A full table with other datasets and more ablation experiments are in Appendix~\ref{apdx:aoi_exp}.


\subsection{Analyzing Auxiliary Option Injection}
\label{sec:aoi_anal}
\input{B_Tables/aoi_ablation}

\paragraph{The choice of extra option affects performance.}
While our main experiments used ``I don't know'' as the extra answer choice, we also tested two alternatives: ``None of the above'' and ``I know the answer.'' Table~\ref{tbl:aoi_anal} shows these results, where ``None'' refers to ``None of the above'' and ``Know'' refers to ``I know the answer''.

The extra option generally helps Llama-3 and Bloomz models - it improves their accuracy and reduces bias compared to the baseline. However, ``I don't know'' works best in most cases. Results differ for the Mistral model: using ``I know the answer'' actually hurts performance and increases bias. See Appendix~\ref{apdx:aoi_exp} for complete results across all datasets and additional experiments.

% \paragraph{More auxiliary options have mixed effects on performance.}
% We find that controlling the number of auxiliary options has notable impact on performance.
% That is, we tried adding multiple auxiliary options, all with the same I-don't-know content.
% In most cases in Table~\ref{tbl:aoi_anal}, adding more auxiliary options did not help improve performance.
% Interestingly, however, both question answering and debiasing performance of Llama-3 significantly improved when using more options.
% This seems to be a peculiar property of Llama-3 that we can improve its performances by simply using multiple auxiliary options.
% Experiments on other datasets are in Appendix~\ref{}.


% \paragraph{Location of the auxiliary option does not decide performance.}
% Another factor to consider is the location of the auxiliary option.
% In our main experiments, we have appended the IDK option to the end of the choice list.
% In comparison, we try placing it in the first choice option (\textit{i.e.}, choice `A'), corresponding to `First Choice AOI' in Table~\ref{tbl:aoi_anal}.
% Overall, there were mixed results, indicating that the location of the auxiliary option is not a decisive factor in determining performance.



==> 5_Analyses/bnp_old.tex <==
\subsection{Analyzing Bias Node Pruning}
\label{sec:bnp_anal}
\paragraph{BNP is not sensitive to the number of nodes pruned.}
Figure~\ref{fig:bnp_analysis}(a) reveals how the performance metrics change as the number of pruned nodes varies.
Regardless of the number of nodes pruned from 8 to 128, our method improves the base performance (dashed lines in the figure) by great margins.
While our method is robust to the number of nodes pruned, searching for the adequate level of pruning may achieve better debiasing performance on the downstream task.
Full list of the figure is provided in Appendix~\ref{apdx:bnp_fig}.

\paragraph{The average bias vector can be generalized across datasets.} 
% If there truly exists a vector that represents the direction of selection bias, the average bias vector retrieved from a dataset should be generalizable to different datasets.
% Considering that the average bias vector represents the direction of selection bias in the embedding space, we evaluate whether it can be generalized across datasets.
The average bias vector represents the direction of selection bias in the embedding space.
If the bias vector captures pure information about selection bias, it should generalize across datasets.
To test this hypothesis, we used the bias vector from one dataset on another.
Figure~\ref{fig:bnp_analysis}(b) shows a heatmap of the improvement in each performance metric.
Interestingly, there is no diagonal pattern, indicating bias vectors retrieved from one dataset can reduce selection bias in other datasets.
For instance, the bias vector from the ARC-Challenge dataset improves the CKLD value of the CSQA dataset by 36$\%$, which is even higher than the 22$\%$ improvement using the bias vector retrieved from its own CSQA dataset.

% , showing that the average bias vector can be generalized to different data distributions as well.


==> 6_RelatedWorks/relatedworks_old.tex <==
\section{Related Works}
\label{sec:relworks}
\paragraph{Selection Bias.}
The large language models' tendency to favor choices in a certain order or with a specific symbol has been discussed in many previous works.
Some of the works investigated the skewed pattern of responses for MCQs~\citep{zheng2024large, wei2024unveiling, pezeshkpour2024large}, emphasizing that selection bias is a critical problem.
Many works have approached this problem by calibrating the output probabilities~\citep{wang2023large, zheng2024large, reif2024beyond, wei2024unveiling, pezeshkpour2024large, wang2024my, balepur2024artifacts, li2024anchored, gupta2024changing},
while others change the way queries are input~\citep{li2023split, robinson2023leveraginglargelanguagemodels}.
Additional approaches include debiasing the LLM through distillation training~\citep{liusie2024teacher} and training the model to enforce its multiple choice symbol binding~(MCSB) property~\citep{xue2024strengthened}.
% Overall, most works approach this problem through calibration, input modification, or supervised fine-tuning.
% Our Bias Node Pruning, on the other hand, introduces a novel approach of parameter pruning in the context of the selection bias.
While parameter pruning methods are often used for efficient deep learning~\citep{srinivas2015data,han2015deep,zhu2017prune,molchanov2019importance,molchanov2022pruning} or to have the LLM unlearn certain factual knowledge~\citep{liu2024model, pochinkov2024dissecting}, parameter pruning has rarely been discussed for debiasing. 
Thus, our Bias Node Pruning is a novel approach in the context of the selection bias.

\paragraph{Auxiliary Options.}
%An interesting discussion of our Auxiliary Option Injection technique is its relationship to human behaviors.
Inclusion of the ``I don’t know” option can improve the quality of data collected in surveys~\citep{schuman1996questions} but does not meaningfully impact the labels assigned by annotators~\citep{beck2022improving}. Recent research has drawn attention to the similarities between surveys, labeling tasks, and model responses to MCQs~\citep{tjuatja2023llms, eckmanposition, 2409.16022}
Further research into LLMs' response behavior would benefit from incorporating insights from the survey science domain: see the discussion in~\citep{eckmanposition}.


% Removing parameters in neural networks has been a commonly done in machine learning literature.
% Many of the works utilized parameter pruning to compress model sizes while preserving performance~\citep{srinivas2015data,han2015deep,zhu2017prune,molchanov2019importance,molchanov2022pruning}.
% Some recent works have leveraged this approach to unlearn factual knowledge~\citep{liu2024model, pochinkov2024dissecting}.


% \vspace{-2mm}
% \paragraph{Data Annotation.}
% One closely related application of selection bias debiasing is data annotation.
% Many works discussed ways to leverage LLMs for automated annotation~\citep{he2024annollm,eckmanposition}, or devised human-machine collaborative frameworks~\citep{li2023coannotating}.
% We expect our work to benefit such annotation systems by reducing the selection bias in answering MCQs.

==> 7_Conclusion/conclusion_claude.tex <==
\section{Conclusion}
When LLMs answer multiple-choice questions, selection bias is a critical problem. Our work makes four key contributions: (1) uncovering the internal mechanisms of selection bias through embedding-level analysis, (2) developing two complementary debiasing methods - Bias Node Pruning (BNP) and Auxiliary Option Injection (AOI), and (3) introducing Choice Kullback-Leibler Divergence (CKLD) as a new metric for measuring selection bias.

BNP and AOI 
%significantly 
reduce selection bias while improving accuracy across diverse MCQ datasets and model architectures. On the ARC-Challenge dataset, combining our methods with existing techniques improves Llama-3's performance by 33.8\%. The methods work effectively for both white-box and black-box models, showing broad applicability.

Looking ahead, several important research directions emerge: (1) investigating how selection bias varies across different model architectures and training procedures, (2) analyzing the relationship between selection bias and other forms of model bias, and (3) developing more general debiasing techniques that can address multiple types of bias simultaneously.

\section*{Limitations}
While our work provides effective methods for mitigating selection bias, fundamental questions remain about its root causes. Key open questions include:
\begin{itemize}
    \item What characteristics of training data contribute to selection bias?
    \item Why do different model architectures exhibit different patterns of selection bias?
    \item How does selection bias relate to the broader question of how LLMs select next tokens?
\end{itemize}
Understanding these questions is crucial not only for addressing selection bias but also for developing more reliable and unbiased language models.

\section*{Ethics Statement} 
This work advances ethical AI development in several ways:
\begin{itemize}
    \item Improving fairness by reducing systematic biases in model outputs
    \item Enhancing transparency through detailed analysis of internal model behavior
    \item Contributing to more reliable and valid automated decision-making
\end{itemize}

While our methods effectively reduce selection bias, we emphasize the importance of continued vigilance regarding other potential biases and ethical considerations in AI systems. Future work should examine how selection bias interacts with other forms of model bias and develop comprehensive approaches to ensuring fair and unbiased AI systems.
